SiPPing Neural Networks: Sensitivity-informed Provable Pruning of Neural Networks

We introduce a pruning algorithm that provably sparsifies the parameters of a trained model in a way that approximately preserves the model's predictive accuracy. Our algorithm uses a small batch of input points to construct a data-informed importance sampling distribution over the network's parameters, and adaptively mixes a sampling-based and deterministic pruning procedure to discard redundant weights. Our pruning method is simultaneously computationally efficient, provably accurate, and broadly applicable to various network architectures and data distributions. Our empirical comparisons show that our algorithm reliably generates highly compressed networks that incur minimal loss in performance relative to that of the original network. We present experimental results that demonstrate our algorithm's potential to unearth essential network connections that can be trained successfully in isolation, which may be of independent interest.

==> drafts/sipp.tex <==
\section{Sensitivity-informed Provable Pruning}
\begin{figure*}[htbp!]
  \centering
   \includegraphics[width=0.9\textwidth]{figures/method-overview}
  %\vspace{-0.5ex}
  \caption{
  The overview of our method consisting of 4 parts. We use a small batch of input points to quantify the relative contribution (importance) of each edge to the output of each neuron. We then construct an importance sampling distribution over the incoming edges and sample a small set of weights for each neuron. The unsampled parameters are then discarded to obtain the resulting compressed network, which has significantly fewer edges than the original network.
  }
  \label{fig:method-overview}
\end{figure*}

In this section, we present and detail the main steps of our pruning algorithm, \textsc{SiPP}, and present its corresponding theoretical guarantees. The outline of our algorithm is shown in Fig.~\ref{fig:method-overview} and the organization of this section is as follows. First, we consider the simplified problem of pruning the incoming edges of a single neuron (i.e., perceptron sparsification) and outline how SiPP can be invoked to provably prune the incoming edges and establish the corresponding sampling complexity. Next, we generalize this per-neuron application of \textsc{SiPP} to all of the neurons in a layer, and establish layer-wise guarantees. Finally, building on the per-layer results, we show via a careful error propagation analysis that if \textsc{SiPP} is invoked to sparsify the incoming edges for every neuron in the network, then the output of the entire network will be approximately preserved.

\subsection{Algorithm Overview}


\subsection{Pruning Edges of a Single Neuron}
Positive edges (and guarantees for the positive part)

\subsection{Pruning a Layer}
Having both pos. and negative edges... Introduce delta for rel error. Layer-wise guarantee lemma

\subsection{Composition: Pruning the Entire Network}

Intuition for how errors propagate at an intuitive level...

Main theorem for 

\subsection{Optimal Sample Allocation}




==> misc/commands.tex <==
% % Comment commands.


%                           %
%                           %
%   GENERAL      COMMANDS   %
%                           %
%                           %
\newcommand{\paragraphsmall}[1]{\textbf{{#1} $\;$}}


%                           %
%                           %
%   GENERAL MATH COMMANDS   %
%                           %
%                           %

\newcommand{\sipp}{\textsc{SiPP}\xspace}
\newcommand{\sippdet}{\textsc{SiPPDet}\xspace}
\newcommand{\sipprand}{\textsc{SiPPRand}\xspace}
\newcommand{\sipphybrid}{\textsc{SiPPHybrid}\xspace}
\newcommand{\sippsimple}{\textsc{SiPPSimple}\xspace}

\newcommand{\size}[1]{\nnz{#1}}
% \newcommand{\nnz}[1]{\mathrm{nnz}(#1)}
\newcommand{\nnz}[1]{\|{#1}\|_0}
\DeclareMathOperator*{\1}{\mathbbm{1}}
\newcommand{\compl}{\mathsf{c}}
\DeclarePairedDelimiterX{\dotp}[2]{\langle}{\rangle}{#1, #2}
\newcommand{\ramp}[1]{\left [ #1 \right]_+}

%                           %
%                           %
%   	  CONSTANTS   		%
%                           %
%                           %
\newcommand{\kmaxInsideLog}{\eta \, \eta^*}
\newcommand{\kmax}{C}
\newcommand{\kmaxSquared}{\log^2(\kmaxInsideLog)}
\newcommand{\CDef}{3 \, \kmax}

%\newcommand{\logTermInside}[1][\eta^*]{8 \, \eta \, #1 }
\newcommand{\logTermInside}[1][4]{ \rho^* \, #1 }
\newcommand{\logTermInsideAmplif}{32 \, |\PP| \, \tau \, \eta \, \eta^* }

\newcommand{\logTermInsideGeneral}{16 \, |\PP'| \, \eta \, \eta^* }

%\newcommand{\logTerm}[1][\eta^*]{\log \left(\logTermInside[#1] / \delta \right)}
\newcommand{\logTerm}[1][\eta^*]{\log \left({#1} \, \rho / \delta \right)}
\newcommand{\logTermAmplif}{\log \left(\logTermInsideAmplif / \delta \right)}

\newcommand{\logTermGeneral}{\log \left(\logTermInsideGeneral / \delta \right)}

\newcommand{\kappaDef}{\sqrt{2 \lambdaStar} \left(1 + \sqrt{2 \lambdaStar} \logTerm \right)}
\newcommand{\kappaDefAmplif}{\sqrt{2 \lambdaStar} \left(1 + \sqrt{2 \lambdaStar} \logTermAmplif \right)}

\newcommand{\kappaDefGeneral}{\sqrt{2 \lambdaStar} \left(1 + \sqrt{2 \lambdaStar} \logTermGeneral \right)}

\newcommand\lambdamax{\log(\eta \, \eta^*)/2}
\newcommand{\lambdaStar}{\lambda_*}
\newcommand{\xmax}{X_\mathrm{max}}
\newcommand{\SizeOfS}[1][]{K \logTerm[#1] }

\newcommand{\SizeOfSAmplif}{\ceil*{\logTermAmplif \kmax}}

\newcommand{\SizeOfSGeneral}{\ceil*{\logTermGeneral \kmax}}


\newcommand{\tauDef}{\ceil*{\frac{\log(4 \, \eta / \delta)}{\log(10/9)}}}

\newcommand{\SizeOfT}{\ceil*{8 \log \left( 8 \, \tau \,  \eta / \, \delta\right) }}


\newcommand\BigO{\mathcal{O}}
\newcommand\Bigo{\BigO}
\newcommand\supp{\mathrm{supp}(\DD)}

\newcommand{\PRIME}[1]{#1^\prime}
\newcommand{\dotP}[2]{#1 \cdot #2}

\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\newcommand{\relu}[1]{\phi(#1)}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\hf}{\frac{1}{2}}
\newcommand{\dd}{{\mathrm{D}}}
\renewcommand{\AA}{{\mathcal{A}}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\iid}{\stackrel{i.i.d.}{\sim}}
\newcommand{\norm}[1]{\left\| #1\right\|}                               %
\newcommand{\br}[1]{\left\{#1\right\}}
\newcommand{\alignspace}{\qquad \qquad}

\newcommand{\abs}[1]        {\left| #1 \right|}
\newcommand{\sq}{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\newcommand{\eps}{\ensuremath{\varepsilon}}                       % Epsilon
\renewcommand{\epsilon}{\varepsilon}

\newcommand{\REAL}{\ensuremath{\mathbb{R}}}                       % Norm
\newcommand{\RR}{{\REAL}}
\newcommand{\median}{\texttt{Median}}
\DeclareMathOperator*{\E}{\mathbb{E} \,}
\let\Pr\relax
\DeclareMathOperator*{\Pr}{\mathbb{P}}
\DeclareMathOperator*{\Var}{\text{Var}}
\newcommand{\V}{\Var}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand{\inprod}[1]{\left\langle #1 \right\rangle}
\newcommand{\eqdef}{\mathbin{\stackrel{\rm def}{=}}}
\DeclareMathOperator*{\rank}{\text{rank}}
\DeclareMathOperator*{\sign}{\text{sign}}

%                           %
%                           %
% PROJECT SPECIFIC COMMANDS %
%                           %
%                           %
% \declaretheorem[name=Theorem]{theorem}
%\declaretheorem[name=Definition]{definition}
%\declaretheorem[name=Assumption]{assumption}
% \declaretheorem[name=Problem]{problem}
% \declaretheorem[name=Example]{example}
%\declaretheorem[name=Corollary, numberlike=theorem]{corollary}
%\declaretheorem[name=Lemma, numberlike=theorem]{lemma}
% \declaretheorem[name=Proposition, numberlike=theorem]{proposition}
% \declaretheorem[name=Remark, numberlike=theorem]{remark}
% \declaretheorem[name=Claim, numberlike=theorem]{claim}
% \declaretheorem[name=Observation, numberlike=theorem]{observation}

\newenvironment{itemizeAlg}{\begin{itemize}[topsep=1pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]}{\end{itemize}}


\renewcommand{\index}{i}
\newcommand{\indexSet}{[s_1^\ell] \times [s_2^\ell] \times [c^\ell]}
\newcommand{\tuple}{(\tupleNoP)}
\newcommand{\tupleNoP}{h,g,r}
% In reality, the following \neuron should be the tuple index i
\newcommand{\neuron}{r}
\newcommand{\edge}{j}
\newcommand{\idx}{k}
\newcommand{\weight}{u}
\newcommand{\layers}{[L]}
\newcommand{\hiddenlayers}{[L-1]}
\newcommand{\given}{\, \mid \, }
\newcommand{\givenRealiz}{\given \realiz(\cdot), \xx}
\newcommand{\givenRealizZLemOne}{\given \xx, \EE_\ZZ}
\newcommand{\givenRealizZ}{\givenRealizZNoEps, \condGood}
\newcommand{\givenRealizZCompl}{\given \realiz(\cdot), \EE_\ZZ^\compl}

\newcommand{\condAmplif}{\EE_{\GG(\Point)}}
\newcommand{\condAmplifDef}{\EE_{\ZZ(\Point)} \cap \EE_{\Delta(\Point)}}

\newcommand{\condGood}{\EE_{\nicefrac{1}{2}}}
\newcommand{\condGoodDef}{\hat{a}(\Point) \in (1 \pm \nicefrac{1}{2}) a(\Point) \qquad \forall{\hat{a}(\cdot) \in \hat \AA^{\ell-1}}}

\newcommand{\givenAmplif}{\given \condAmplif \cap \EE^{\ell-1} }

\newcommand{\givenAmplifCompl}{\given \condAmplif^\compl \cap \EE^{\ell-1} }

\newcommand{\givenRealizSub}{\given \hat{a}^{\ell-1}(\cdot), \, \Point}

\newcommand{\realiz}{\mathbf{ a}}

\newcommand{\compressiblelayers}{[L]}
\newcommand{\etaDef}{\sum_{\ell = 1}^L \eta^\ell}
\newcommand{\etaStarDef}{\max_{\ell \in \compressiblelayers} \eta^{\ell}}

\newcommand{\ComputationTime}{\Bigo \left( \eta \, \, \eta^* \, \log \big(\eta \, \eta^*/ \delta \big) \right)}

\newcommand{\ComputationTimeGeneralized}{\Bigo \left( \eta \, \, \eta^* \, \log \big(\eta \, \eta^* \, |\PP'| / \delta \big) \right)}



\newcommand{\epsilonStar}{\epsilon_*}

\newcommand{\epsilonDenomContant}{2}
\newcommand{\epsilonPrimeDef}{\frac{\epsilon}{\epsilonDenomContant \, (L-1)}}

\newcommand{\epsilonLayer}[1][\ell]{\epsilon_{#1}}
\newcommand{\epsilonLayerDef}[1][\ell]{\frac{ \epsilon'}{ \DeltaNeuronHatLayers[#1]}}
\newcommand{\epsilonLayerDefWordy}[1][\ell]{\frac{ \epsilon}{\epsilonDenomContant \, (\LayersCompressed) \DeltaNeuronHatLayersDef[#1]}}


%\newcommand{\SampleComplexity}[1][\epsilonLayer]{\ceil*{\frac{(6 + 2\epsilon) \SNeuron \kmax \log ({{#1} / \delta}) }{\epsilon^2}}}
\newcommand{\SampleComplexity}[1][\epsilonLayer]{\ceil*{(6 + 2\epsilon) \, \SNeuron \, \kmax \, \log ({{#1} / \delta}) \epsilon^{-2}}}

\newcommand{\SampleComplexityDeltaEach}[1][\epsilonLayer]{\ceil*{\ (6 + 2{#1}) \Delta_r^2  \, \left(\sum_{\edge \in \Wpm} s_\edge\right) \, \kmax \, \log ({8 \, \eta / \delta}) \epsilon^{-2}}}

\newcommand{\SampleComplexityDelta}[1][\epsilonLayer]{(7 + 2{#1}) \Delta_r^2 \, \SNeuron_r \, \kmax \, \log ({8 \, \eta / \delta}) \epsilon^{-2}}

% \newcommand{\SampleComplexityDeltaLayers}[1][\epsilonLayer]{\ceil*{\frac{ 32  (L - 1) \, (\Delta_r^{\ell \rightarrow})^2 \left(\sum_{\edge \in \Wpm} s_\edge\right) \kmax \log ({8 \eta / \delta}) }{{#1}^2}}}
%\newcommand{\SampleComplexityDeltaLayers}[1][\epsilonLayer]{\ceil*{\frac{ 32  (L-1)  (\Delta_r^{\ell \rightarrow})^2  \kmax \log (8 \eta / \delta) \sum_{\edge \in \Wpm} s_\edge }{{#1}^2}}}

\newcommand{\SampleComplexityDeltaLayers}[1][\epsilonLayer]{\ceil*{32  \, L^2 (\Delta_r^{\ell \rightarrow})^2 \, \kmax \log (8 \eta / \delta) \,  \epsilon^{-2} \, \sum_{\edge \in \Wpm} s_\edge }}

\newcommand{\epsilonNeuron}[1][\mNeuron]{\sqrt{\frac{\tilde S}{{#1}} \left(\frac{\tilde S}{{#1}} + 6\right)} + \frac{\tilde S}{{#1}}}

\newcommand{\epsilonNeuronOpt}[1][\mNeuron]{\sqrt{\frac{\tilde S_r}{{#1}} \left(\frac{\tilde S_r}{{#1}} + 6\right)} + \frac{\tilde S_r}{{#1}}}

\newcommand{\epsilonNeuronDeterministic}[1][\mNeuron]{3 K \sum_{\edge \in (\II \setminus \II_{{#1}})} s_j}

\newcommand{\SampleComplexityWordy}{\frac{ L^2 \, (\Delta^{\ell \rightarrow})^2 \, \SNeuronWordy \, \kmax \, \log (\eta / \delta) }{\epsilon^2}}


% \newcommand{\SampleComplexityWordy}{\frac{33  \, (\LayersCompressed)^2 \, (\Delta_r^{\ell \rightarrow})^2 \, \SNeuronWordy \, \kmax \, \log (8 \, \eta / \delta) }{\epsilon^2}}

\newcommand{\SampleComplexityGeneral}{\ceil*{\frac{32  \, (\LayersCompressed)^2 \, (\DeltaNeuronHatLayers)^2 \, \SNeuronWordy \, \kmax \, \log (16 \, |\PP'| \, \eta / \delta) }{\epsilon^2}}}

\newcommand{\SampleComplexityGeneralConcise}[1][\epsilonLayer]{\ceil*{\frac{8  \, \SNeuron \, \kmax \log ({16  |\PP'| \, \eta / \delta}) }{{#1}^2}}}

\newcommand{\SampleComplexityAmplif}[1][\epsilonLayer]{\ceil*{\frac{8  \, \SNeuron \, \kmax \log ({32  |\PP| \, \tau \, \eta / \delta}) }{{#1}^2}}}


\newcommand{\LayersCompressed}{L}
\newcommand{\epsilonPrime}{\frac{\epsilon}{2 \, (\LayersCompressed)}}

\newcommand{\param}{\theta}
\newcommand{\paramDef}{(\WW^1, \ldots, \WW^L)}
\newcommand{\paramHat}{\hat{\theta}}
\newcommand{\paramHatDef}{(\WWHat^1, \ldots, \WWHat^L)}

\newcommand{\ComputationTimeSum}[1]{\sum_{\ell = #1}^L \eta^{\ell-1} \eta^{\ell}}

\newcommand{\f}{f_\param}
\newcommand{\fHat}{f_{\paramHat}}

\newcommand{\Input}{x}
\newcommand{\Label}{y}
\newcommand{\Point}{\Input}
\newcommand{\PointPrime}{\Input'}
\newcommand{\xx}{\mathbf{\Input}}

\newcommand{\pos}{\mathrm{pos}}
\newcommand{\negg}{\mathrm{neg}}
\newcommand{\InputPos}{\Input_\pos}
\newcommand{\InputNeg}{\Input_\mathrm{neg}}


\newcommand{\Wpm}{\II}
\newcommand{\Wplus}{\II_+}
\newcommand{\Wminus}{\II_-}
\newcommand{\WplusDefVerbose}{\{\edge \in  \II : w_\edge > 0\}}
\newcommand{\WminusDefVerbose}{\{\edge \in  \II: w_\edge < 0 \}}
\newcommand{\WplusDef}{\WplusDefVerbose}
\newcommand{\WminusDef}{\WminusDefVerbose}


\newcommand{\II}{\mathcal{I}}

% \newcommand{\gDef}[1]{\max_{a(\cdot) \in \AA^{\ell-1}} \, \frac{\WWRowCon_\edge \, a_{\edge}(#1)}{\sum_{\idx \in \II } \WWRowCon_\idx \, a_{\idx}(#1) }}
\newcommand{\gDefNoMax}[2][a]{ \frac{\WWRowCon_\edge \, {#1}_{\edge}(#2)}{\sum_{\idx \in \II_i^\ell } \WWRowCon_\idx \, {#1}_{\idx}(#2) }}
\newcommand{\gDefNoMaxNice}[2][a]{ \nicefrac{\WWRowCon_\edge \, {#1}_{\edge}(#2)}{\sum_{\idx \in \II_i^\ell } \WWRowCon_\idx \, {#1}_{\idx}(#2) }}

\newcommand{\gDef}[2][a]{\max_{{#1}(\cdot) \in \AA_i^\ell} \gDefNoMax[{#1}]{#2}}
\newcommand{\gDefNice}[2][a]{\max_{{#1}(\cdot) \in \AA_i^\ell} \gDefNoMaxNice[{#1}]{#2}}

\newcommand{\gHatDef}[1]{\max_{a(\cdot) \in \AA^{\ell-1}} \, \frac{\WWRowCon_\edge \, \hat a_{\edge}(#1)}{\sum_{\idx \in \II} \WWRowCon_\idx \, \hat a_{\idx}(#1) }}

\newcommand{\g}[1]{g_\edge(#1)}
\newcommand{\gHat}[1]{\hat g_\edge(#1)}

\newcommand{\cdf}[1]{F_\edge \left(#1 \right)}
\newcommand{\cdfHat}[1]{\hat F_\edge \left(#1 \right)}


% for pseudo-code only
\newcommand{\sPM}[1][\edge]{s_{#1}}
\newcommand{\mPM}{m}
\newcommand{\qPM}[1]{q_{#1}}


\newcommand{\mNeuron}{N}
\newcommand{\mNeuronWordy}{\mNeuron_r}
\newcommand{\mPos}{m^+_\neuron}
\newcommand{\mNeg}{m^-_\neuron}
\newcommand{\SNeuron}{S}
\newcommand{\SNeuronWordy}{S_\neuron^\ell}
\newcommand{\STildeDef}[2][S]{\frac{{#1} C}{3} \log ({{#2} / \delta)}}
\newcommand{\SPos}{\SNeuronWordy{^+}}
\newcommand{\SNeg}{\SNeuronWordy{^-}}
\renewcommand{\S}{S}

\newcommand{\T}[1][]{T_{#1}}
\newcommand{\TTilde}[1][]{\widetilde{T}_{#1}}
\newcommand{\TMinTilde}[1][]{\tilde{T}^-_{#1}}

\newcommand{\bound}{M}


\newcommand{\WWRow}[1][\neuron]{w_{#1}}
\newcommand{\WWHatRow}[1][\neuron]{{\hat{w}_{#1}}}
\newcommand{\WWRowCon}[1][\neuron]{w}
\newcommand{\WWHatRowCon}[1][\neuron]{{\hat{w}}}
\newcommand{\WWHat}{\hat{\WW}}

\newcommand{\err}[2][\Point]{\mathrm{err}_{\index}(#2, #1)}
\newcommand{\errDef}[1][\Point]{\abs{\frac{\hat z_\index (#1)}{z_\index(#1)} - 1}}

\newcommand{\errTil}[2][\Point]{\widetilde{\mathrm{err}}_{\index}(#2, #1)}

\newcommand{\errPlus}[1][\Point]{\errTil[#1]{\WWHatRowCon^+}}
\newcommand{\errPlusDef}[1][\Point]{\abs{\frac{\hat z_\index^+ (#1)}{\tilde z_\index^+(#1)} - 1}}

\newcommand{\errMinus}[1][\Point]{\errTil[#1]{\WWHatRowCon^-}}
\newcommand{\errMinusDef}[1][\Point]{\abs{\frac{\hat z_\index^- (#1)}{\tilde z_\index^-(#1)} - 1}}


\newcommand{\errRatio}{\frac{\WWHatRowCon^\ell \, \hat{a}^{\ell-1}(\Point)}{\WWRowCon^\ell \, a^{\ell-1}(\Point)}}


\newcommand{\errRatioPlus}[1][\Point]{\frac{\sum_{\idx \in \Wplus} \WWHatRowCon_\idx \, \hat{a}_\idx(#1) }{\sum_{\idx \in \Wplus} \WWHatRowCon_\idx \, \hat{a}_\idx(#1)}}

\newcommand{\errRatioMinus}[1][\Point]{\frac{\sum_{\idx \in \Wminus} \WWHatRowCon_\idx \, \hat{a}_\idx(#1) }{\sum_{\idx \in \Wminus} \WWHatRowCon_\idx \, \hat{a}_\idx(#1)}}

\newcommand{\EErr}[1]{\E_{{#1}, \, \Point \given \hat{a}^{l-1}(\cdot) }}

\newcommand{\ErrCondRand}{\WWHatRowCon^\ell \givenRealizSub}

\newcommand{\ErrCondRandPlus}{\WWHatRowCon^{+} \givenRealizSub}
\newcommand{\ErrCondRandMinus}{\WWHatRowCon^{-} \givenRealizSub}

\newcommand{\DeltaNeuronSample}[1][\xx']{\hat{\Delta}_\index^{\ell}(#1)}

\newcommand{\DeltaNeuron}[1][\Point]{\Delta_\index^{\ell}(#1)}

\newcommand{\DeltaNeuronHat}[1][\ell]{\hat \Delta^{#1}}

\newcommand{\DeltaNeuronHatLayers}[1][\ell]{\DeltaNeuron[#1 \rightarrow]}

\newcommand{\DeltaNeuronHatDef}[1][\Point']{\left(\frac{1}{|\SS|} \max_{\index \in \indexSet} \, \sum_{#1 \in \SS} \DeltaNeuron[{#1}]\right) + \kappa}

\newcommand{\DeltaNeuronHatLayersDef}[1][\ell]{\prod_{k=#1}^L \DeltaNeuronHat[k]}

\newcommand{\DeltaNeuronTrue}{\Delta_\index^{\ell}}
\newcommand{\DeltaNeuronDef}[1][{\Point}]{\frac{z_\index^+(#1) + z_\index^-(#1)}{|z_\index(#1)|}}

\newcommand{\DeltaNeuronTrueDef}[1][\xx]{ \frac{\sum_{\idx \in [\eta^{\ell-1}]}  |\WWRow[\neuron \idx]^\ell \, a_\idx^{\ell-1}(#1)|} {\left|\sum_{\idx \in [\eta^{\ell-1}]} \WWRow[\neuron \idx]^\ell \, a_\idx^{\ell-1}({#1})\right|}}


\newcommand{\Wpl}{\Wplus}
\newcommand{\Wmi}{\Wminus}
\newcommand{\s}[1][\edge]{s_{#1}}


\newcommand{\SPlu}{S_+}
\newcommand{\SMin}{S_-}
\newcommand{\CC}{\mathcal C}
\newcommand{\SNeu}{S^{\ell}_\neuron}

\newcommand{\G}{\Gamma}
\newcommand{\DD}{{\mathcal D}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\ZZ}{{\mathcal Z}}

\newcommand{\FF}{{\mathcal F}}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\YY}{\mathcal{Y}}
\newcommand{\WW}{W}


% % Expectation with respect to coreset C
\newcommand{\EPlu}{\E \nolimits_{\CC \given \hat a(\cdot), \, \Point}\,}

% % Variance with respect to coreset C
\newcommand{\VarCond}{\Var \nolimits_{\CC \given \hat a(\cdot), \, \Point}\, }

% % Expectation with respect to coreset C
\newcommand{\EPluLemOne}{\E \nolimits_{\CC \givenRealizZLemOne}\,}

% % Variance with respect to coreset C
\newcommand{\VarCondLemOne}{\Var \nolimits_{\CC \givenRealizZLemOne}\, }

\newcommand\Reals{\mathbb{R}}
\newcommand\PP{\mathcal{P}}
\renewcommand\QQ{\mathcal{Q}}
\renewcommand\SS{\mathcal{S}}
\newcommand\MM{\mathcal{M}}
\newcommand\LLL{\mathcal{L}}
\newcommand\GG{\mathcal{G}}
\newcommand\TT{\mathcal{T}}
\newcommand\BB{\mathcal{B}}

\DefineFNsymbols{mySymbols}{{\ensuremath\dagger}  {\ensuremath\ddagger} *\P
   *{**}{\ensuremath{\dagger\dagger}}{\ensuremath{\ddagger\ddagger}}}
\setfnsymbol{mySymbols}

%\newcommand{\smallsubsub}[1]{\vspace{-1.5ex}\subsubsection*{#1}\vspace{-1.5ex}}

\newcommand{\smallsubsub}[1]{\subsubsection*{#1}}



==> misc/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> misc/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
% hyperref makes hyperlinks in the resulting PDF.
\usepackage{hyperref}
\usepackage{xr-hyper}

\usepackage{algorithm}
\usepackage{algorithmic}
% customize comments for algorithmic
\renewcommand{\algorithmiccomment}[1]{ $\quad\triangleright$ #1}

\usepackage[export]{adjustbox}
\usepackage{subcaption}
\usepackage[percent]{overpic}
\usepackage{wrapfig}
\usepackage{graphicx}
\usepackage{svg}

\usepackage{caption}
\captionsetup{font=small}
\captionsetup[sub]{font=small}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{float}

% Comment this out for final
%\usepackage{amsmath,amsfonts,amsthm,amssymb, nccmath}
\usepackage{amsmath,amsfonts,amsthm,amssymb, nccmath}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\allowdisplaybreaks % allow page breaks of equations
\usepackage{bbm}
\usepackage{framed}
\usepackage{enumerate}
\usepackage{mathtools}
\usepackage{scalefnt}
\usepackage{changepage}

\usepackage{comment}
\usepackage{setspace}
\usepackage{verbatim}
\usepackage{xcolor}
\usepackage{scalefnt}
%\usepackage{xr}

\usepackage[shortlabels]{enumitem}
\setlist{nolistsep, noitemsep, leftmargin=20pt, labelwidth=3pt}

\usepackage{placeins}
\usepackage{color}
\usepackage{footmisc}
\usepackage{xspace}

%\usepackage{thmtools}
%\usepackage{thm-restate}

\usepackage{multirow}
\usepackage{booktabs}
\usepackage{array}
\usepackage{tabularx}

% FROM ICML
\usepackage{microtype}



==> sec/impact.tex <==
\section*{Broader Impact Statement}
The present work aims at broadening the applicability of deep learning systems. This is achieved with regard to two aspects, certifiability and computational performance. By proposing a novel pruning technique, we reduce the computational requirements of evaluating neural networks which helps with their deployment on systems that impose a computational or energy budget. That is, network pruning simplifies deployment of networks on resource constrained devices, such as phones, watches, and in time critical applications such as control systems. By proposing provable guarantees for our method,  we also aim to enable the use of neural networks in applications that require formal certifiability i.e. in safety critical scenarios or for decision support in health. The provided guarantees focus on the pruning problem, one of many building blocks in a  learning pipeline. However, our  methodology has the potential to be adapted for the theoretical analysis of other aspects of deep learning. 

==> shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
%\PassOptionsToPackage{numbers, sort, square}{natbib}
%\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\include{misc/preamble}
\include{misc/commands}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{problem}{Problem}
\newsiamremark{assumption}{Assumption}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{SiPPing Neural Networks}{}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{SiPPing Neural Networks: Sensitivity-informed Provable Pruning of Neural Networks\thanks{Submitted to the editors 11/28/2020.
\funding{This research was supported in part by the U.S. National Science Foundation (NSF) under Awards 1723943 and 1526815, Office of Naval Research (ONR) Grant N00014-18-1-2830, Microsoft, and JP Morgan Chase.}}}

% Authors: full names plus addresses.
\author{Cenk Baykal$^*$\thanks{MIT CSAIL, Cambridge, MA 
  (\email{baykal@mit.edu}, \email{lucasl@mit.edu}, \email{igilitschenski@mit.edu}, \email{rus@mit.edu})} 
\and Lucas Liebenwein$^*$\footnotemark[2]
\and Igor Gilitschenski\footnotemark[2]
\and Dan Feldman\thanks{Robotics and Big Data Laboratory, University of Haifa, Israel (\email{dannyf.post@gmail.com}) \newline$^*$These authors contributed equally to this work.}
\and Daniela Rus\footnotemark[2]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "main"
%%% End: 

